CCPrefix: Counterfactual Contrastive Prefix-Tuning for Many-Class Classification

Recently, prefix-tuning was proposed to efficiently adapt pre-trained language models to a broad spectrum of natural language classification tasks. It leverages soft prefix as task-specific indicators and language verbalizers as categorical-label mentions to narrow the formulation gap from pre-training language models. However, when the label space increases considerably (i.e., many-class classification), such a tuning technique suffers from a verbalizer ambiguity problem since the many-class labels are represented by semantic-similar verbalizers in short language phrases. To overcome this, inspired by the human-decision process that the most ambiguous classes would be mulled over for each instance, we propose a brand-new prefix-tuning method, Counterfactual Contrastive Prefix-tuning (CCPrefix), for many-class classification. Basically, an instance-dependent soft prefix, derived from fact-counterfactual pairs in the label space, is leveraged to complement the language verbalizers in many-class classification. We conduct experiments on many-class benchmark datasets in both the fully supervised setting and the few-shot setting, which indicates that our model outperforms former baselines.

==> approach.tex <==
\section{Approach}
In this section, we describe in detail our approach, whose overall architecture is shown in \Cref{fig:model}.

\subsection{Contrastive Prompts Construction} \label{sec:CPfC} In this section, we would elaborate the process of exploiting all possible contrastive attributes from each instance, and the way we construct the prompt templates.

\subsubsection{Contrastive Attributes Construction} \label{sec:att_generation}
In the light of the social science's view, humans rely on exploring contrastive attributes between the objective factual and their potential counterfactuals for classification \citep{miller2019}.
Thus, for tasks with finite label space, following \citep{jacovi2021contrastive}, we prune the finite label space to construct all causal factors by projecting the sentence representation into the contrastive space. 
First of all, each instance $x$ would be encoded by a deep neural encoder $f(\cdot)$ that transforms $x$ into $\mX = \{\ve_1, \ve_2, \ldots, \ve_l\} \in \R^{l \times d_e}$, where $l$ is the sentence length and $d_e$ the embedding dimension.
Then, we use a multi-layer perception (MLP) with ReLU activation, and mean pooling over the sequence to get the whole sentence representation, $\vh_x = \meanpool(\mlp(\mX))$.

Commonly, for classification, the prediction of the model $\mW \vh_x$ is linear in the latent input representation. The processor of prediction is aim to map $\vh_x$ to a specific direction $\vw_i$ via dot product to obtain the logits of class $i$.
As proposed by \citet{jacovi2021contrastive} in terms of contrastive explanation, given two classes, $y_p$ and $y_q$, if we are particularly interested in the contrastive attributes that the model predicts $y_p$ rather than $y_q$, we can construct a new basis, $\vu_{p,q} = \vw_{p} - \vw_{q}$, which represents a \textit{contrastive space} for $y_p$ and $y_q$. Thus, $y_p$ is the fact while $y_q$ is one of its counterfactuals.
However, for each instance, the golden label is unavailable before prediction. Hence, we hypothesize that the $i$-th class $y_i$ is the fact in turn while the rest in the finite-label space are counterfactuals to build fact-counterfactual pairs.
Specifically, we employ the derivable vectors as the verbalizer $\mV \in \R^{|R| \times d_e}$ to map to the class set $\gY$.
Thus, supposing that $i$-th class $y_i$ is the fact while one of the rest class $y_j$ is the counterfactual, the contrastive subspace is:
\begin{align}
    \vu_{i,j}=\vv_i - \vv_j \in \R^{d_e}, i \in |R|, j \neq i \label{eq:subspace}
\end{align}
Then, by projecting the instance representation $\vh_x$ onto the subspace $\vu_{i,j}$, we can explore the contrastive attributes between the fact-counterfactual pair:
\begin{align}
    \vc_{i,j} = \frac{\vu_{i,j} \otimes \vu_{i,j}^\top}{\langle \vu_{i,j}^\top \vu_{i,j} \rangle}\ \vh_x \label{eq:project}
\end{align}
where $\otimes$ is the outer product and $\langle \cdot \rangle$ is the inner product.
For the contrastive attributes generated between the same fact and the rest counterfactuals, we denote these attributes as $\mC_{i,*} \in \R^{(|R|-1) \times d_e}$, where $i,*$ represents the fact-counterfactual pairs consisting of the $i$-th fact and the rest labels assumed as counterfactuals.
Sequentially operating eq.\ref{eq:subspace} and eq.\ref{eq:project}, we extract all contrastive attributes $\mC \in \R^{|R| \times (|R|-1) \times d_e}$ from each instance.
We summarize the former procedure of constructing contrastive attributes in Algorithm \ref{alg:CAC}.

% For each instance $x$, assuming that the $i$-th class $y_i$ is the fact while the other $y_{i,*}$ are counterfactuals,
% we employ the derivable vectors as the verbalizer $\mV \in \R^{|R| \times d_e}$ to map to the class set $\gY$. Thus, contrastive space is:
% \begin{align}
%     \mU_{i,*} = \vv_i - \mV_{i,*} \in \R^{(|R|-1) \times d_e},
% \end{align}
% where $\vv_i$ is the $i$-th component and $\mV_{i,*
% }$ is the remaining matrix in $\mV$, excluding its $i$-th component. 
% Then, by projecting the sentence representation $\vh_x$ onto $\mU_{i,*}$, we can yield contrastive attributes for $i$-th class.
% Following \citet{jacovi2021contrastive}, we define the contrastive transformation to be the orthogonal projection onto each subspace for each instance:
% \begin{align}
%     \mC_{i,*} = \frac{\mU_{i,*} \otimes \mU_{i,*}^\top}{\langle \mU_{i,*}^\top \mU_{i,*} \rangle}\ \vh_x
% \end{align}
% where $\otimes$ is the outer product and $\langle \cdot \rangle$ is the inner product.
% $\mC_{i,*}$ captures the contrastive attributes between the fact $i$-th classes and all the other counterfactuals. Each row $\vc_{i,j}$ is the contrastive evidence between the fact $i$-th class and the specific counterfactual $j$-th class.
% Thus, we obtain all possible contrastive evidences $\mC=\{\mC_{1,*}, \ldots, \mC_{|R|,*}\} \in \R^{|R| \times (|R|-1) \times d_e}$ by looping over the class label $i$.

% 引入prototype的内容，要解释清楚为什么需要prototype, 如何训练prototype
Obviously, since we suppose each label as the fact to form fact-counterfactual pairs in turn, it is inevitable to face the noisy attributes projected by invalid fact-counterfactual pairs for each instance.
% not all exploited contrastive attributes are correct because there is only one accurate fact in the finite label space. 
% Concretely, contrastive attributes generated by the subspaces between the instance's ground-truth label and the other labels are valid while the other contrastive attributes are 
Therefore, the contrastive attributes should be selected only if it is generated by the valid fact-counterfactual pairs formed by the accurate label.
To distinguish valid contrastive attributes, we introduce a set of global prototypes $\{\mP_{0,*}, \mP_{1,*}, \ldots, \mP_{|R|,*}\} \in \R^{|R| \times (|R|-1) \times d_e}$ corresponding to contrastive attributes.
Concretely, for the contrastive attributes $\vc_{i,j}$ generated by projecting instance onto the subspace between $i$-th fact and $j$-th counterfactual, there is only one corresponding prototype $\vp_{i,j}$.
The fine-grained global prototypes can learn the common features of its corresponding fact-counterfactual attribute among the whole training instances.
During training, according to the instance's ground-truth label, these prototypes can be split into two groups.
One is the set of positive prototypes while the other is the rest negative prototypes $\mP_{-,*} \in \R^{(|R|-1) \times (|R|-1) \times d_e}$.
The positive prototypes represent the common knowledge of the corresponding attributes $\mC_{+,*}$ generated by the valid fact-counterfactual pairs. 
These prototypes are trained with the following self-contrastive learning loss:
\begin{align}
    \gL_{\rm con} = -\log \frac{\exp(\langle \mW \mC_{+,*}, \mP_{+,*} \rangle)}{\sum_- \exp(\langle \mW \mC_{+,*}, \mP_{-,*} \rangle))} \label{eq:con_loss}
\end{align}
where $\mW \in \R^{d_e \times d_e}$ is the learning weight matrix and $\langle \cdot \rangle$ is the inner product to calculate the similarity. 
% This objective forces global prototypes to lie at the center of their attributes for counterfacutals. 
This objective forces the positive prototypes draw up the positive contrastive attributes. Simultaneously, the negative contrastive attribtues would be pushed away from the positive prototypes. 
Thus, by calculating the similarities between instance's contrastive attributes and the corresponding prototypes, we select the top-$m$'s most similar attributes $\mC_{sel} \in \R^{m \times d_e}$ as additional prompt tokens to fill into the original prompt template $T(\cdot)$, as shown in \Cref{fig:proto_illustration}. 

% Although the aforementioned contrastive learning framework can learn distinguishable prototypes, the semantic features from the text are needed to construct prompt tokens. This is achieved by selecting relevant contrastive attributes based on these prototypes. 
% Specifically, by calculating the similarities between attributes and its corresponding prototypes, $\langle \mW \mC_{i,*}, \mP_{i,*} \rangle$, we select the most prominent top-$m$ attributes $\mC_{sel}$ as additional prompt tokens to fill into the original prompt template $T(\cdot)$, as shown in \Cref{fig:proto_illustration}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/c_selection.pdf}
    \caption{An illustration of the selection process of top-2 contrastive attributes $\vc_{i,j}$ using the similarities between all possible $\vc_{i,j}$ and their corresponding prototypes $\vp_{i,j}$, where $i$-th class is fact and $j$-th class is its counterfactual.}
    \label{fig:proto_illustration}
\end{figure}

\subsubsection{Prompt Template} \label{sec:prompt_con}
In general, we insert the selected contrastive attributes to the original prompt template. It is worth noting that since the selected contrastive attributes are continuous vectors, we first embed the instance and original prompt tokens and then combine them together in the following form: 
\begin{equation}
\begin{aligned}
    T(\mX, \mC)=\{&\ve_1, \ldots, \ve_l, \\
    &\textcolor{blue}{\vc_1, \ldots, \vc_m}, \\
    &\ve_{t_1}, \ldots, \ve_{t_n}, \ve_{\texttt{[MASK]}}\}, 
\end{aligned}
\end{equation}
where $\{\ve_1, \ldots, \ve_l\}$
is the embedding of instance $\mX$, $\{\vc_1, \ldots, \vc_m\}$ is the additional prompt tokens for the selected contrastive attributes, $\{\ve_{t_1}, \ldots, \ve_{t_n}\}$ is the embedding of original prompt tokens and $\ve_{\texttt{[MASK]}}$ is the embedding of \texttt{[MASK]} for filling in the answer token from the verbalizer.

\subsection{Siamese Prompt Tuning} \label{sec:siames}
We note that some selected top-$m$ contrastive attributes may inevitably take false classes as facts, thereby introducing unwanted noise. 
Therefore, it is crucial to force the PLMs to focus on the valid contrastive attributes and consequently stabilize the model performance.
Hence, we leverage a simple Siamese representation learning method \citep{chen2021exploring} to simultaneously train the PLMs, $\gM$, via maximizing the similarity between the prompt templates with selected contrastive attributes $\mC_{sel}$ and the same instance with all positive attributes $\mC_{+,*}$. 
These two inputs with different contrastive attributes are fed into $\gM$ to obtain the \texttt{[MASK]} representation $\vz$ and $\vz_+$:
\begin{equation}
\begin{aligned}
    \vz = \gM(\hat{\mX})=T(\mX, \mC_{sel}), \\
    \vz_+ = \gM(\hat{\mX}_+)=T(\mX, \mC_{+,*}).
\end{aligned}
\end{equation}
Then, we minimize the negative cosine similarity between two outputs with an MLP $f(\cdot)$:
\begin{align}
    \gD(\vz, \vz_+) = - \frac{f(\vz)}{||f(\vz)||_2} \cdot \frac{\vz_+}{||\vz_+||_2}
\end{align}
Following \citet{chen2021exploring}, we use a symmetrized loss with the stop-gradient operation:
\begin{align}
    &\gL_{\rm s} \!=\! \frac{1}{2}\gD(f(\vz), \stopgrad(\vz_+)) \!+\! \frac{1}{2}\gD(f(\vz_+), \stopgrad(\vz)). \label{eq:sym_loss}
\end{align}
Here, $\mX$ with attributes $\mC_{+,*}$ receives no gradient from $\vz_+$ in the first term, but it receives gradients from $f(\vz_+)$ in the second term, and vice versa. 

% Finally, the output logit for each class is given by the inner product between $f(\vz)$ and the verbalizer $\mV$, which is trained with 
% \begin{align}
%     \gL_{\rm cls} = - \sum_{i=1}^{|R|} {\rm log} p(y_i = \vv_i|x), \label{eq:ins_loss}
% \end{align}
% where the probability score is given by
% \begin{align}
%     p(y_k = \vv_k|x) = \frac{\exp (f(\vz) \cdot \vv_k )}{\sum_{j} \exp (f(\vz) \cdot \vv_j )}.
% \end{align}

Finally, the learning objective is to minimize the following loss:
\begin{align}
    \gL_{\rm cls} = - \frac{1}{|\gX|} \sum^{|\gX|}_{k=1} {\rm log} p(\texttt{[MASK]}=\vv_k | x_k) \label{eq:ins_loss}
\end{align}
where $p(\texttt{[MASK]}=v_k | x_k)$ is the predicted distribution for the $k$-th sample in dataset $\gX$ and $\vv_k$ is the answer word corresponding to its ground truth label $y_k$.

Overall, our final training loss is
\begin{align}
    \gL = \gL_{\rm cls} + \gL_{\rm s} + \gL_{\rm con}
\end{align}


==> conclusion.tex <==
\section{Conclusion}
In this paper, we propose a novel task-agnostic approach named CCPrompt that could incorporate contrastive counterfactuals for many-class classification tasks.
We sequentially construct fact-counterfacutal pairs as the basis of the contrastive spaces to extract contrastive attributes from the sample. With a set of global prototypes, the model can select relevant contrastive attributes from the current instance context, and later insert them into the original prompt. During training, we use a simple Siamese representation learning on the augmented prompts for model stabilization, hence making them free from supervised labels.
% We train a set of global prototypes to align the corresponding attributes for each instance.
% According to the similarity between attributes and prototypes, we select top-$m$ attributes as additional tokens in prompts for inference. During training, we further select positive attributes for siamese representation learning.
% To heuristically select valid attributes as addition tokens of the prompt template, we train a set of global prototypes that aligns the corresponding contrastive attributes for each instance. 
% To force PLMs focusing on the valid contrastive attributes that generated with actual fact, we employ a simple siamese representation learning for the instance with two different prompt templates. One is the selected contrastive attributes while the other is the positive attributes with actual class as fact.
The experiment results verify the superiority of our model without extra data and human experts for manually designing prompt templates. 
While we have shown that our method is flexible enough for a wide range of tasks in NLP, leveraging contrastive explanations in logic reasoning tasks remains an unveiled challenge for future work. 

==> experiments.tex <==
\section{Experiments}
We conduct comprehensive experiments on several many-class classification tasks, including relation classification (RC), topic classification (TC) and entity typing (ET), to exhibit the superiority of CCPrompt. 

\subsection{Datasets} 
We adopt 4 popular datasets for relation classification, including TACRED \citep{zhang2017position}, TACREV\citep{alt2020tacred}, ReTACRED \citep{stoica2021re} and SemEval 2010 Task 8 \citep{hendrickx2009semeval} (SemEval). One dataset for topic classification is DBPedia \citep{lehmann2015dbpedia}, and one entity typing dataset is FewNERD \citep{ding2021few}. 

\begin{itemize}
    \item \textbf{TACRED} is one of the largest and most widely used datasets for relation classification.
    
    \item \textbf{TACREV} is built based upon the original TACRED dataset. The authors correct the errors in the original development and the test set of TACRED, while the training set is left intact.
    
    \item \textbf{ReTACRED} is another revised version of TACRED. The authors refactored the training, development, test set and a few relation types.
    
    \item \textbf{SemEval} is a traditional dataset for relation classification.
    
    \item \textbf{DBPedia} is an ontology dataset with structured information extracted from WikiPedia. We privately set a 10\% of the training dataset as the validation set.
    
    \item \textbf{FewNERD} is a manually large-scale, fine-grained dataset of entity typing containing 66 fine-grained entity types. In our work, we only consider the inter task, where train/dev/test splits may share coarse-grained types while keeping the fine-grained entity types mutually disjoint.
\end{itemize}
    
More details of these datasets are shown in \Cref{tab:dataset_stats}. 
For evaluation, we use $F_1$ scores as the metric for RC, and mean accuracy for TC and ET.
% 这里要确认一下DBPedia的数据拆分要求
\begingroup
\renewcommand{\arraystretch}{1.1}
\begin{table}[ht]
    \small
    \centering
    \setlength\tabcolsep{3pt}
    % \resizebox{\textwidth}{15mm}{XXXX}
    \begin{tabular}{lccccc}
        \toprule     
        Dataset  & \#Class & Task & $|\gD_{\rm train}|$ & $|\gD_{\rm dev}|$ & $|\gD_{\rm test}|$\\
        \midrule
        TACRED & 42 & RC & 68,124 & 22,631 & 15,509 \\
        TACREV & 42 & RC & 68,124 & 22,631 & 15,509 \\
        ReTACRED & 40 & RC & 58,465 & 19,584 & 13,418 \\
        SemEval & 19 & RC & 6,507 & 1,493 & 2,717 \\
        DBPedia & 14 & TC & 56,000 & \multicolumn{1}{c}- & 70,000 \\
        FewNERD & 66 & ET & 338,753 & 48,667 & 96,901 \\
        \bottomrule
    \end{tabular}
    \caption{Basic statistics of the datasets, where RC stands for relation classification, TC stands for topic classification, and ET stands for entity typing.}
    \label{tab:dataset_stats}
\end{table}
\endgroup


\begingroup
\renewcommand{\arraystretch}{1.1}
\begin{table*}[ht]
    \small
    \centering
    \begin{tabular}{lccccc}
        \toprule
        % \multicolumn{5}{c}{Fully Supervised Setting} \\
        % \midrule
         & Extra Data & TACRED & TACREV & ReTACRED & SemEval \\
        \midrule
        C-GCN \citep{zhang2018graph} & - & 66.3 & 74.6 & 80.3 & - \\
        $\text{\textsc{RoBERTa}}_{\textsc{LARGE}}$ \citep{liu2019roberta} & - & 68.7 & 76.0 & 84.9 & 87.6 \\
        \textsc{KnowBERT} \citep{peters2019knowledge} & $\checkmark$ & 71.5 & 79.3 & - & 89.1 \\
        \textsc{SpanBERT} \citep{joshi2020spanbert} & $\checkmark$ & 70.8 & 78.0 & 85.3 & - \\
        \textsc{LUKE} \citep{yamada2020luke} & $\checkmark$ & \textbf{72.7} & 80.6 & 90.3 & - \\
        PTR \citep{han2021ptr} & - & 72.4 & 81.4 & 90.9 & 89.9 \\
        \midrule
        CCPrompt (Ours) & - & 72.6 & \textbf{82.9} & \textbf{91.2} & \textbf{90.6} \\
        \midrule
        w/o ConAtt in \S \ref{sec:att_generation} & - & 70.0  & 80.9 & 90.6 & 90.1 \\
        w/o Prototypes in \S \ref{sec:att_generation} & - & 71.9 & 81.2 & 90.5 & 90.4 \\
        w/o $\gL_{\rm con}$ in Eq.\ref{eq:con_loss}  & - & 71.3 & 81.8 & 90.6 & 90.2 \\
        w/o Siamese in \S \ref{sec:siames} & - & 72.0 & 81.8 & 90.8 & 90.1 \\
        \bottomrule
    \end{tabular}
    \caption{$F_1$ scores (\%) for RC tasks on the 4 datasets in the fully supervised setting. ``w/o ConAtt'' denotes using manually prompt template and soft verbalizer. ``w/o Prototypes'' denotes that the cluster is rely on the verbalizer. ``w/o Siamese'' denotes that the input of prompts template only maintain instance and selected contrastive attribute.}
    \label{tab:fullysupervised}
\vspace{10pt}
\end{table*}
\endgroup


\begingroup
\renewcommand{\arraystretch}{1.1}
\begin{table*}[ht]
    \small
    \centering
    \begin{tabular}{lccccccccc}
        \toprule
        % \multicolumn{10}{c}{Few-Shot Setting in Relation Classification (RC)} \\
        % \midrule
         & \multicolumn{3}{c}{TACRED} & \multicolumn{3}{c}{TACREV} & \multicolumn{3}{c}{ReTACRED} \\\cmidrule(lr){2-4}
        \cmidrule(lr){5-7}
        \cmidrule(lr){8-10}
          & 8 & 16 & 32 & 8 & 16 & 32 & 8 & 16 & 32 \\
        \midrule
        Fine-Tuning (Ours) & 12.2 & 21.5 & 28.0 & 13.5 & 22.3 & 28.2 & 28.5 & 49.5 & 56.0 \\
        PTR \citep{han2021ptr} & 28.1 & 30.7 & 32.1 & 28.7 & 31.4 & 32.4 & 51.5 & 56.2 & 62.1 \\ 
        \midrule
        % GenPT (BART) & 29.7 & 33.5 & 35 & 29.6 & 32.9 & 34.3 & 50.6 & 56.7 & 62.1 \\
        % GenPT (T5) & 28.2 & 32.1 & 35 & 29.7 & 31.7 & 34.6 & 52.4 & 57.3 & 62.3 \\
        % \midrule
        CCPrompt (Ours) & \textbf{30.1} & \textbf{33.4} & \textbf{37.6} & \textbf{29.8} & \textbf{33.0} & \textbf{34.0} & \textbf{54.5} & \textbf{61.4} & \textbf{65.2} \\
        \midrule
        w/o ConAtt in \S \ref{sec:att_generation} & 18.1 & 29.6 & 32.6 & 18.1 & 29.0 & 32.7 & 41.1 & 55.5 & 64.1\\
        w/o Prototypes in \S \ref{sec:att_generation} & 28.5 & 33.1 & 36.3  & 30.4 & 31.7 & 33.2 & 54.2 & 56.3 & 62.1 \\
        w/o $\gL_{\rm con}$ in Eq.\ref{eq:con_loss} & 28.2 & 33.2 & 37.3 & 28.9 & 32.1 & 33.8 & 53.5 & 59.7 & 64.4 \\ 
        w/o Siamese in \S \ref{sec:siames} & 23.8 & 33.1 & 32.9 & 27.9 & 30.4 & 33.2 & 50.6 & 57.7 & 63.4 \\
        \bottomrule
    \end{tabular}
    \caption{$F_1$ scores (\%) for RC tasks in the few-shot setting. We use $K=8, 16, 32$ for few-shot settings.}
    \label{tab:fs_rc}
\vspace{10pt}
\end{table*}
\endgroup

% \subsection{Settings and Implementation Details}
\subsection{Settings} To fairly compare with SoTA baselines, we evaluate CCPrompt in both fully supervised and few-shot settings for RC tasks. For TC and ET, we evaluate CCPrompt only in few-shot setting, where for each class, $K$ instances are sampled for training and validation.
Following previous works \cite{han2021ptr, cui2022prototypical}, we set $K$ as 8, 16, 32 for relation classification and 1, 2, 4, 8, 16 for topic classification and entity typing. 
It is worth noting that we use a fixed set of 5 random seed to sample instances and take the average of all results as the final result.

\subsection{Implementation Details} Our model is implemented based on PyTorch \citep{paszke2019pytorch} and the Transformer repository of Huggingface \citep{wolf2020transformers}.
For a fair comparison, we follow settings of previous works. 
For RC and TC tasks, our model is based on $\text{\textsc{RoBERTa}}_{\textsc{LARGE}}$, while for ET, it is based on $\text{\textsc{BERT}}_{\textsc{base}}$. The optimizer is Adam for all datasets, where the learning rate is manually tuned $\in\{$1$e$-5, 3$e$-5, 5$e$-5 $\}$, and the decay rate is set to 1$e$-2, and the batch size is set to 16.
For the fully-supervised setting, the epoch is 5 while for few-shot setting, it is 30.
The best model is selected based on the performance on the development set. In both training and inference, we select top-$m$ attributes for prompts, where $m=|R|-1$.

\subsection{Comparison Methods}
We mainly compare CCPrompt with several representative methods in many-class classification tasks, including learning-from-scratch methods, fine-tuning methods and prompt-tuning methods. 
    1) C-GCN \citep{zhang2018graph} is a learning-from-scratch based on graph neural networks for relation classification.
    2) For fine-tuning vanilla PLMs, we directly select $\text{\textsc{RoBERTa}}_{\textsc{LARGE}}$ as our baselines for relation classification.
    3) Since entity information is crucial in relation classification, we select \textsc{SPANBERT} \citep{joshi2020spanbert}, \textsc{KnowBERT} \citep{peters2019knowledge} and LUKE \citep{yamada2020luke} as our baselines.
    4) We select PTR \citep{han2021ptr}, a prompt augmentation model, for relation classification.
    5) For topic classification and entity typing, our baselines are ProtoVerb \citep{cui2022prototypical} that uses manual prompts, and PETAL \citep{schick2020automatically} that extracts words as prompts.
    % (6) We compare with PETAL \citep{schick2020automatically}, which finds the words that maximize the likelihood of the training data.

\begingroup
\renewcommand{\arraystretch}{1.1}
\begin{table*}[ht]
    \small
    \centering
    \caption{Few-Shot TC \& ET performance of $F_1$ scores (\%) on the DBPedia and FewNERD datasets. We use $K=1, 2, 4, 8, 16$ for few-shot settings.}
    \label{tab:fs_tcet}
    \begin{tabular}{lcccccccccc}
        \toprule
        % \multicolumn{11}{c}{Few-Shot Setting in Topic Classification (TC) \& Entity Typing (ET)} \\
        % \midrule
         & \multicolumn{5}{c}{DBPedia} & \multicolumn{5}{c}{FewNERD} \\
        \cmidrule(lr){2-6}
        \cmidrule(lr){7-11}
         & 1 & 2 & 4 & 8 & 16 & 1 & 2 & 4 & 8 & 16 \\
        \midrule
        PETAL \citep{schick2020automatically} & 60.06 & 78.21 & 86.40 & 88.41 & 92.90 & 20.88 & 31.28 & 43.10 & 50.78 & 55.49 \\
        ProtoVerb \citep{cui2022prototypical} & 72.85 & 85.49 & 90.91 & 95.75 & 96.30 & \textbf{25.00} & \textbf{35.72} & 48.28 & 56.06 & 61.29 \\
        \midrule
        CCPrompt (Ours) & \textbf{84.02} & \textbf{93.26} & \textbf{95.17} & \textbf{97.66} & \textbf{98.45} & 22.78 & 32.47 & \textbf{51.49} & \textbf{58.54} & \textbf{63.38} \\
        \bottomrule
    \end{tabular}
\end{table*}
\endgroup

\subsection{Main Quantitative Evaluation}
In this part, we compare CCPrompt with several recent methods to provide comprehend analysis. In few-shot setting, we mainly compare with prompt-tuning based model for relation classification, topic classification and entity typing to show the superiority and universality of CCPrompt.

% Fully supervised setting
\subsubsection{Fully Supervised Setting} Obviously, in \Cref{tab:fullysupervised}, CCPrompt achieves significant improvements than former baselines, and even outperforms \textsc{KnowBERT} and LUKE that leverage external task-specific knowledge to enhance models.
Compared with PTR \citep{han2021ptr} that manually construct logic rules as the prompt, CCprompt extracts the task-related information from each instance to form the unique prompts. 
Such comparison indicates that the unique task-related information from each instance can better stimulate task-specific knowledge in PLMs.


% Few-shot setting
\subsubsection{Few-Shot Setting} To further prove the robustness of our model, we evaluate CCPrompt in few-shot settings. 
For relation classification, as shown in \Cref{tab:fs_rc}, CCPrompt outperforms PTR by a large margin. Especially, for ReTACRED, our model surpasses by 6.6\% on average. 
It is worth noting that PTR manually designs the task-specific sub-rules to construct prompts, which is a prompt augmentation model. 
Meanwhile, the prompt in CCPrompt provides specific distinguishable features of each instance to point out the crucial difference between several classes, which directly stimulates the PLMs in data scarce scenarios.
For topic classification, as shown in the left panel of \Cref{tab:fs_tcet}, CCPrompt exceeds PETAL and ProtoVerb by a large margin.
% PETAL finds the words that maximize the likelihood of the training data. ProtoVerb learns prototype vectors as verbalizer by contrastive learning. Both methods employ the manual prompts. 
Specifically, in the extreme data scarce scenario ($K=1, 2$), our model surpasses ProtoVerb by 15.3\% and 9.1\%. This demonstrates that, if the class labels are semantically diverse, our model is capable of acquiring sufficient knowledge from the PLM even in this limit.
% our model can better explore the class-related features and stimulate specific knowledge from PLMs via contrastive prompts.
% 一样的soft verbalizer. 一个是由contrastive learning学出来的，一个是由contrastive explanation生成的prompt 
% 突出verbalizer和prompt比较关键， 
% 对于class之间语义区分明显的任务而言，
For entity typing, our model exceeds former baseline in several scenarios ($K=4, 8, 16$) but not good when training instances are extremely scarce ($K=1, 2$). 
% As to what reason it is, we deduce that FewNERD is a fine-grained entity typing dataset, where the difference between classes is subtle. For example, under type ``building'', there are ``building-theater'', ``building-library'', ``building-hotel'' and so on.
We infer that for fine-grained entity typing, although our model can cancel out most of the attributes between two classes sharing the same coarse class with subtle differences in semantic (e.g., `building-theater'' and ``building-library'' are under type ``building''), it is hard to discriminate such contrastive attributes in extreme data scarce scenario, especially without prior knowledge.
% Thus, without sufficient training samples, it is difficult for CCPrompt to discriminate them. 

% In a nutshell, the pre-training phrase enables PLMs to comprehend complex semantics, prompts for classification tasks needs to provide explicit class-differentiate features for forcing PLMs focus on class-
% and ignore the class-irrelevant information.

\subsection{Ablation Study}
To further analyze the potency of each component in CCPrompt, we conduct an ablation study on relation classification datasets.
As shown in the bottom panel of \Cref{tab:fullysupervised} and \Cref{tab:fs_rc}, the performance of the model degrades to various degrees. It is worth noting that ``w/o ConAtt'' causes more performance degradation in the few-shot setting than in the fully supervised one, which indicates that contrastive attributes can further stimulate the knowledge for classification in PLMs.
For ``w/o Prototypes'', we use the similarities between the attributes and the verbalizers as the selection criteria instead.
Obviously, the performance of ``w/o Prototypes'' has significantly decreased in both settings. 
Comparing with prototypes-based criteria, the coarse grained criteria introduces more noise attributes, leading to the performance degradation.
Thus, it is crucial to set global prototypes for implicit clustering to learn the common features of each contrastive attribute among training instances.
% Since the intra-class attribute factors are generated via various counterfacts, the attribute factors are too discrete to cluster only via the answer words of verbalizer.
``w/o $\gL_{\rm con}$'' has less performance reduction in few-shot setting than that in fully supervised setting. We infer that the unbalanced training data distribution may hurt the performance significantly. Besides, it is worth noting that our contrastive attribute construction is irrespective of any entity information. Thus, the attributes may be too dispersed in embedding space, hence failing to clustering around the prototypes.
Although only slightly underperformed in the fully supervised setting, the performance of ``w/o Siamese'' drops severely in the extreme data scarce scenario ($K=8$), indicating that simple representation learning can force the PLMs to focus on the valid contrastive attributes in prompts.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.85\textwidth]{figures/CaseAnalysis.pdf}
%     \caption{\small The similarity distribution of the same sentence with different query. The first is its ground truth label \textit{per:city\_of\_birth} and the second is the contrastive space between the ground truth label and the counterfactual \textit{per:city\_of\_death}.}
%     \label{fig:casestudy}
% \end{figure*}


\begingroup
\renewcommand{\arraystretch}{1}
\begin{table}[t]
    \centering
    \small
    \caption{The top selected counterfactual relation learned by the model for some relation types.}
    \label{tab:top_counterfact}
    \begin{tabular}{ll}
    \toprule
        \multicolumn{1}{l}{Relation} & \multicolumn{1}{l}{Top selected counterfact} \\
        \hline
        \textit{per:siblings} & \textit{per:title}  \\
        % \textit{per:spouse} & \textit{org:shareholders} \\
        \textit{per:parents} & \textit{per:countries\_of\_residence}  \\
        % \textit{org:top\_members/employees} & \textit{org:members}  \\
        \textit{org:dissolved} & \textit{org:member\_of }  \\
        \textit{per:origin} & \textit{org:dissolved}  \\
        \textit{per:children} & \textit{per:country\_of\_birth}  \\
        % \textit{org:political/religious\_affiliation} & \textit{per:parents}  \\
        \textit{per:city\_of\_birth} & \textit{per:city\_of\_death}  \\
        \textit{per:employee\_of} & \textit{per:countries\_of\_residence}  \\
        \textit{per:religion} & \textit{per:city\_of\_death}  \\
        \textit{org:alternate\_names} & \textit{org:founded\_by}  \\
        \textit{per:cause\_of\_death} & \textit{per:country\_of\_death} \\
        \textit{org:website} & \textit{org:members} \\
    \bottomrule
    \end{tabular}
\end{table}
\endgroup

\begin{figure*}[ht]
\small
\centering%
\begin{tabular}{p{\dimexpr0.49\textwidth-1.1\tabcolsep-\arrayrulewidth\relax}|p{\dimexpr0.49\textwidth-1.1\tabcolsep-\arrayrulewidth\relax}}
\toprule
\multicolumn{1}{c}{\textit{y$^*$=per:city\_of\_birth}} & \multicolumn{1}{|c}{\textit{(y$^*$, y')=per:city\_of\_birth, per:city\_of\_death}} 
\\
\cmidrule{1-2} 
\ttfamily\colorbox{my_color!48.55253571192018}{Gross} \colorbox{my_color!0}{,} \colorbox{my_color!0}{a} \colorbox{my_color!100.0}{60-year-old} \colorbox{my_color!0}{native} \colorbox{my_color!0}{of} \colorbox{my_color!46.5177842050648}{\underline{Potomac}} \colorbox{my_color!0}{,} \colorbox{my_color!0}{Maryland} \colorbox{my_color!0}{,} \colorbox{my_color!0}{was} \colorbox{my_color!0}{working} \colorbox{my_color!0}{for} \colorbox{my_color!0}{a} \colorbox{my_color!0}{firm} \colorbox{my_color!0}{contracted} \colorbox{my_color!0}{by} \colorbox{my_color!0}{USAID} \colorbox{my_color!43.65155763583778}{when} \colorbox{my_color!0}{\underline{he}} \colorbox{my_color!0}{was} \colorbox{my_color!0}{arrested} \colorbox{my_color!0}{Dec} \colorbox{my_color!0}{3} \colorbox{my_color!0}{,} \colorbox{my_color!0}{2009} \colorbox{my_color!0}{,} \colorbox{my_color!0}{and} \colorbox{my_color!0}{sent} \colorbox{my_color!0}{to} \colorbox{my_color!0}{Cuba} \colorbox{my_color!0}{'s} \colorbox{my_color!87.51506855363964}{high-security} \colorbox{my_color!0}{Villa} \colorbox{my_color!76.3718455390458}{Marista} \colorbox{my_color!53.505618969818755}{prison} \colorbox{my_color!0}{.} 

  &
\ttfamily
\colorbox{my_color!0}{Gross} \colorbox{my_color!0}{,} \colorbox{my_color!0}{a} \colorbox{my_color!0}{60-year-old} \colorbox{my_color!99.99999999999999}{native} \colorbox{my_color!77.05655042958857}{of} \colorbox{my_color!0}{\underline{Potomac}} \colorbox{my_color!0}{,} \colorbox{my_color!0}{Maryland} \colorbox{my_color!0}{,} \colorbox{my_color!0}{was} \colorbox{my_color!0}{working} \colorbox{my_color!0}{for} \colorbox{my_color!0}{a} \colorbox{my_color!0}{firm} \colorbox{my_color!95.78406437745862}{contracted} \colorbox{my_color!73.01442004090212}{by} \colorbox{my_color!0}{USAID} \colorbox{my_color!0}{when} \colorbox{my_color!0}{\underline{he}} \colorbox{my_color!0}{was} \colorbox{my_color!0}{arrested} \colorbox{my_color!0}{Dec} \colorbox{my_color!0}{3} \colorbox{my_color!0}{,} \colorbox{my_color!0}{2009} \colorbox{my_color!0}{,} \colorbox{my_color!0}{and} \colorbox{my_color!0}{sent} \colorbox{my_color!0}{to} \colorbox{my_color!0}{Cuba} \colorbox{my_color!0}{'s} \colorbox{my_color!60.13545221225092}{high-security} \colorbox{my_color!0}{Villa} \colorbox{my_color!0}{Marista} \colorbox{my_color!0}{prison} \colorbox{my_color!0}{.}
\\
\bottomrule
\end{tabular}
\caption{The \colorbox{my_color!100}{highlighted} tokens of the same sentence where the two entities are \underline{underscored}. On the left, the tokens are projected onto the ground truth \textit{y$^*$=per:city\_of\_birth}, and on the right onto the contrastive space between \textit{y$^*$} and the counterfactual \textit{y'=per:city\_of\_death}.}
\label{fig:casestudy}
\end{figure*}


\subsection{Reasoning Analysis} \label{sec:reasoning}
% 1. 分析prompts是否正确highlight了句子中的某些部分
    %   这个通过利用内积，将attention值大于th的highlight看看是否可信 (case study)
        % 选择的第15类，其中的contrastive attribute factor是15对34
% 2. 分析verbalizer是否具有正确的含义：没有可解释性！
% 3. 分析几个class中的topk prompts是否是正确的
% a) 确实能选到正确的contrastive attribute factors
% b) prompt-tuning的必要性
In addition, we analyze the efficacy of the underlying prompt tokens in their contrastive explanations' perspective, especially in the following two aspects:
1) Does the prompt tokens correspond to a reasonable fact-counterfact space?
% In this section, we mainly analysis the effectiveness of contrastive explanation prompt tokens via explaining two important problems:
% 1) Does the prompt tokens maintain the correct attribute factors that generated via reasonable contrastive space?   
2) Compared to using only the prompt tokens related to the ground-truth label, does the contrastive attribution highlight more reasonable parts of the sentence for model prediction?
Considering that CCPrompt outperforms the baselines even stronger in the few-shot setting, we pick the ReTACRED dataset in the $K=16$ setting for this analysis.
% Considering its superiority performance in few-shot setting, we analysis the \textcolor{red}{[MODEL]} trained in ReTACRED with 16 training instances per class.

\subsection{Selected Counterfact} Since the prompt tokens are instance aware, we limit our analysis to a subset of 7K instances in the test set that could be correctly classified. For each relation type, we count the most frequently selected counterfactual relation. Part of the results are shown in \Cref{tab:top_counterfact}.
% \paragraph{Quantitative Analysis} In the whole dataset, 24.13\% correctly classified samples have at least one correct attribute factors and only 3.83\% wrongly classified samples maintain correct attribute factors. Thus, combining the performance change in ablation study, it is indicate that such correct attribute factors can directly stimulate PLMs to focus on the classify related information.
% Furthermore, we explore that the contrast space for correct attribute factors is generated via the reasonable counter facts.
It is notable that most of the time the model can match a pair \textit{per} relations, or a pair of \textit{org} relations. Also, the model prefers to select two relation types semantically correlated but with subtle differences.
For example, for relation \textit{per:city\_of\_birth} or \textit{org:dissolved}, the corresponding contrastive attribute factor is \textit{per:city\_of\_death} or \textit{org:member\_of}, respectively.
% in class \textit{per:cause\_of\_death}, the contrastive space for correct attribute factors is constructed by the counter fact \textit{per:country\_of\_death}.

\subsection{Case Study} Moreover, we conduct a case study to qualitatively analyze which tokens in a sentence are highlighted for model prediction, as shown in \Cref{fig:casestudy} for the relation \textit{per:city\_of\_birth} between entity ``\texttt{he}'' and ``\texttt{Potomac}''. 
We compute the similarity of each word in the sentence and the fact \textit{y$^*$=per:city\_of\_birth}, or the contrastive attribution factor between \textit{y$^*$=per:city\_of\_birth} and \textit{y'=per:city\_of\_death}. Finally, for clarity, in both cases we only highlight the words with similarity score that are greater than 1.02 times the average similarity score.
% The first is the similarity between each word and the fact \textit{per:city\_of\_birth} while the second is the similarity between each word and the attribute factor build between the fact \textit{per:city\_of\_birth} and the counter fact \textit{per:city\_of\_death}.
% It is obvious that the first distribution is smoother than the second distribution with a wrong highlight part ``prison''.
% Moreover, the attribute factor can accent the part around word ``native'', which is the direct feature for classification.
In \Cref{fig:casestudy}, we observe that with the contrastive attribute factor between \textit{y$^*$} and \textit{y'}, the highlighted words are relatively concentrated, and contain the key determinant \texttt{``native of''}. On the contrary, only using \textit{y$^*$} will the highlighted texts be more scattered, and misaligned with human expectations of what should be more predictable.

\subsection{Error Analysis \& Limitations}
While we analyze the root causes of incorrect predictions, we observe that
1) if the class labels have subtle differences in their semantics, more data will be needed to construct valid contrastive attributes. Therefore, the model performance may decrease in the extreme data scarce limit, e.g., for FewNED dataset at $K=1,2$. On the other hand, if the class labels are semantically diverse, our model steadily outperforms the baselines in this limit, e.g., for DBPedia dataset. 
% For those tasks with subtle classes, e.g., entity typing, our model is hard to directly prune such finite classes via counterfactual. 
% Besides, for each instance, it may not include sufficient reasoning for those sophisticated counterfactual.
2) For the entity-centric classification tasks, when the sample has multiple entities, it is possible that the selected contrastive attributes are mismatched with the targeting entity, thus leading to misprediction.
% For the classification tasks depending on the entities, e.g., relation classification, our model do not infer the contrastive attributes with respect to the entities' information. Thus, leading to the obtained evidences are not strong related with specific entities.

Then, we mainly discuss the limitations of CCPrompt.
First, it is obvious that our model, CCPrompt, can be only applied in classification tasks. Whatever they are binary, triple or multiple-classes classification tasks, CCPrompt can achieve remarkable performances.
Second, with the increase of the finite-label spaces, both time complexity and spatial complexity would increase exponentially.
Third, the size of PLMs would not affect the equipment of our model, but may affect the performance.

==> intro.tex <==
\section{Introduction}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/intro_example.pdf}
    \caption{An illustrative example of entity typing task from FewNERD \cite{ding2021few} dataset. Option A is its ground-truth label, and Option B is the counterfactual. Red words are the related attributes for the question. 
    % The contrastive attributes for ``Why A not B'' is more effective for model prediction.
    }
    \label{fig:intro_example}
\end{figure}

The prompt-tuning paradigm has achieved great success in natural languages processing (NLP), which can elicit the specific knowledge from pre-trained language models (PLMs) to serve various downstream tasks, e.g., machine translation \citep{liu2021gpt,li2022prompt}, text generation \citep{radford2019language,brown2020language,schick2020few}, relation extraction \citep{han2021ptr}.
Compared to the prevalent \textit{fine-tuning} paradigm, the prompt-tuning paradigm is more flexible and generalizable with fewer learnable parameters by virtue of the introduced prompt templates \citep{brown2020language,trinh2018simple,petroni2019language,davison2019commonsense}. 


% prompt -> multi-class
Regularly, the prompt-tuning paradigm is recognized as a promising solution to narrow the gap of objective forms between pre-training and fine-tuning \citep{brown2020language,schick2020automatically}. 
% For classification tasks, 
When applied to classification tasks, a set of label words is designed as the candidate set for filling into the placeholder (e.g., \texttt{[MASK]}) in carefully-designed prompt template. 
Some works \citep{webson2021prompt,cao2021knowledgeable} have demonstrated that the performance of prompt models is quite sensitive to the choice of label words and the way of template design. 
% 对于few-class classification任务，label words找起来简单
For few-class classification tasks (i.e., categories less than dozens), 
it is relatively tractable for experts to
% due to the mutual exclusive classes in semantic, we can easily 
design the prompt and select the valid label words as there are obvious semantic bounds among the limited number of categorical labels.
For example, in natural language inference, the classes are entailment, neural and contradiction. Some works \citep{schick2020automatically,liu2021gpt} use \{``yes'', ``maybe'', ``no''\} as the set of label words. 
% In binary sentiment classification, the positive sentiment and the negative sentiment are respectively mapped to ``good'' and ``bad''.
In binary sentiment classification, the label words are ``good'' and ``bad''.

% 对于many-class classification的问题，找到合适的prompt和label很难。尤其是关系，type这种类，很难找到合适的answer words。
However, for many-class classification tasks, it is quite challenging to manually select an optimal set of label words, not to mention the semantic overlap existing between classes.
For instance, as shown in Fig \ref{fig:intro_example}, ``Person-Actor'' and ``Person-Employee'' are the common classes in the entity typing task.
% Towards the optimal prompt-tuning, some works \citep{schick2020automatically,shin2020autoprompt,gao2020making,han2021ptr} start to automatically generate prompts and the label words.
% \citet{schick2020automatically} first automatically generates the label words from existing vocabulary with manually designed prompt templates.
% \citet{shin2020autoprompt} utilizes gradient-guided search method to generate both prompt templates and label words.
% \citet{gao2020making} generates several prompt candidates and select one of the most effective ones via the development sets.
Thus, \citet{han2021ptr} manually designs logic rules to merge several sub-prompts together as the final prompt for each class in relation extraction with many classes. 
Since the classes in relation extraction are correlated to both sentence semantics and entity types, the sub-prompts are designed to reflect the sentence semantics and the entity types, respectively. 
The logic rules combine these prompts together to specifically capture the subtle difference among the classes in relation extraction. 
For example, for the relation ``person:employee'', the logic rule restricts that one sub-prompt should determine whether a marked entity is human or not, and the other sub-prompt should determine whether sentence express the semantics of employee.
Despite introducing prior knowledge about tasks and classes, it is time-consuming to manually design the logic rules, which requires extra expert knowledge and makes the prompts only effective for these particular classes. 
Without the logic rules, the model is unable to distinguish the subtle differences among a plenty of categorical labels in many-class classification tasks.

In this paper, for tasks with the finite-label space, we propose Counterfactual Contrastive Prompt-Tuning (CCPrompt) approach to extract the contrastive attributes.
Unlike previous works, for many-class classification tasks, our approach is more universal by avoiding artificial design, and each prompt highlights the unique information of each training instance.

% 先谈insights
Inspired by the research in social science \citep{miller2019}, we introduce the contrastive procedure of human explanation for classification.
Human rely on exploring contrastive attributes \citep{miller2019} between the objective factual and other potential counterfactuals, rather than the explicit evidence of the objective factual.
Concretely, rather than explaining ``why A'', it is more effective to explain ``why A not B'', where B is an implicit counterfactual of A in the current context.
For example, in \Cref{fig:intro_example}, we show an instance from FewNERD \citep{ding2021few} dataset, where humans need to classify the type of Greg. From a machine learning point of view, a well-trained model will recognize that Greg is associated with several attributes, including ``Houston'', ``company'' and ``actor'', all of which are considered useful for prediction. As a result, the similarities among all attributes are high enough so that they are all highlighted. However, from the contrastive explanation perspective, the similarity between Employee or Actor and most of the attributes will be canceled out, leaving only the rest that are effective for model prediction.

% 再谈具体做法
Formally, we first project the representation of each instance onto the subspace spanned by fact-counterfactual label pairs to obtain the corresponding contrastive attributes. 
To prune the finite label space, each label would be assumed as the fact in turn while the other labels would be the counterfactual labels.
Therefore, for each instance, all possible contrastive attributes could be extracted. 
Since the contrastive attributes extracted by wrong fact-counterfactual label pairs are quite noisy, we set up a global prototypes to select the valid contrastive attributes by implicitly learning the common features of valid attributes among training instances. 
Then, the selected contrastive attributes will form the prompt with its instance as the input of PLMs.
To make the training process much more robust, we perform a simple Siamese representation learning with two input. The first input is the prompt with the selected contrastive attributes and the second is the prompt with correct contrastive attributes. 
This learning method can force the PLMs to focus on the valid attributes in prompt.
During inference, only the selected contrastive attributes and the instances will be combined to form the prompts as the input for PLMs.



% 第五段：总结&contribution
To fully verify the effectiveness of CCPrompt, we conduct extensive experiments on three many-class classification tasks in both fully supervised setting and few-shot setting, including relation classification, topic classification and entity typing.
For relation classification, we evaluate our model on four popular datasets: TACRED, TACREV, ReTACRED and SemEval 2010 Task 8 in both fully supervised setting and few-shot setting. For topic classification and entity typing, we evaluate our model on DBPedia and FewNERD respectively only in few-shot setting.
We further exhaustively analyze the reasoning of contrastive attributes and fact-counterfactual pairs. 
% 1t and) Does the prompts include reasonable contrastive attributes?
% 2) Does the contrastive attributes highlight the reasonable parts of the sentence?
Sufficient experimental results indicate that CCPrompt significantly surpasses former baselines. 

==> limitation.tex <==
\section*{Limitations}
In this section, we mainly discuss the limitations of CCPrompt.
First, it is obvious that our model, CCPrompt, can be only applied in classification tasks. Whatever they are binary, triple or multiple-classes classification tasks, CCPrompt can achieve remarkable performances.
Second, the encoder in our model should be Pre-trained Language Models, e.g., \textsc{BERT}, \textsc{RoBERTa}, etc. The size of PLMs would not affect the equipment of our model, but may affect the performance.

==> preliminaries.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/PromptRE_revise.pdf}
    \caption{Our proposed model, CCPrompt. For easy comprehension, we zoom out contrastive prompts for classification \Cref{sec:CPfC} and contrastive evidence generation in \Cref{sec:att_generation}. To generate all contrastive evidence, we assume these classes as the only fact in sequence. The losses $\gL_{\rm cls}$, $\gL_{\rm s}$ and $\gL_{\rm con}$ are defined in \Cref{eq:ins_loss}, \Cref{eq:sym_loss} and \Cref{eq:con_loss}. The black line is the forward 
   path for both training and inference, while the green line is the training path with supervised signal.}
    \label{fig:model}
\end{figure*}

% Adding a algorithm
\begin{algorithm}[t]
    \small
    \renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    \caption{Contrastive Attributes Construction}
    \label{alg:CAC}
    \begin{algorithmic}[1]
        \REQUIRE the class set $\gY$, instance $x$, a PLM model $\gM$
        \ENSURE Contrastive attributes $\mC \in \R^{|R| \times (|R|-1) \times d_e}$
        % \STATE Given the class set $\gY$ and instance's representation $\vh_x$, construct its all possible counterfactual $\mC$ 
        % \STATE |R| = number of the classes in $\gY$
        \STATE Initialize the verbalizer $\mV = \phi(\gY) \in \R^{|R|\times d_e}$
        \STATE Initialize the matrix $\mC \in \R^{|R| \times (|R|-1) \times d_e}$
        \STATE Obtain instance representation $\vh_x = \meanpool(\gM(x)) $
        \FORALL{$\vv_i \in \mV$}
            \FORALL{$\vv_j \in \mV, i \neq j $}
                \STATE Construct the contrastive subspace $\vu_{i,j}=\vv_i - \vv_j \in \R^{d_e}$
                \STATE Project the instance onto the subspace $\vc_{i,j} = \frac{\vu_{i,j} \otimes \vu_{i,j}^\top}{\langle \vu_{i,j}^\top \vu_{i,j} \rangle}\ \vh_x$
            \ENDFOR
            \STATE Form $\mC_{i,*}$ representing the attributes between $i$-th fact and the other label
        \ENDFOR
        \STATE \textbf{return} $\mC \in \R^{|R| \times (|R|-1) \times d_e}$
    \end{algorithmic}
\end{algorithm}


\section{Preliminaries}
Before introducing our model, we first provide the preliminary about the prompt-tuning paradigm for tasks with finite label space, e.g., classification, relation extraction, entity typing.

Formally, the task with the finite-label space can be denoted as $\gT=\{\gX, \gY\}$, where $\gX$ is the instance set, $\gY=\{y_1, y_2, \ldots, y_{|R|}\}$ is the class set, and $|R|$ is the number of classes. 

% \subsection{Contrastive Explanation}\label{sec:contrastive_explnation}
% In general, for classification tasks, each instance $x$ would be encoded by a deep neural encoder $f(\cdot)$ that transforms $x$ into a vector $\vh_x \in \R^d$. 
% On top of that, a linear layer $\mW \in \R^{|R| \times d}$ is used to obtain the logits for the classes. 
% In the end, $\hat{y} = \argmax_{y \in \gY}\mW \vh_x$ is the predicted class of this model, where $\vh_x = f(x)$. 

% Recall that the prediction of the model, $\mW \vh_x$ is linear in the latent input representation. Let $\vw_i$ be the row in $\mW$ corresponding to class $i$. 
% The processor of prediction is actually to map $\vh_x$ to a specific direction $\vw_i$ via dot product to obtain the logits of class $i$.
% As proposed by \citet{jacovi2021contrastive}, given two classes, $y_p$ and $y_q$, if we are particularly interested in the contrastive attributes that the model predicts $y_p$ rather than $y_q$, we can construct a new basis, $\vu_{p,q} = \vw_{p} - \vw_{q}$, which represents a \textit{contrastive space} for $y_p$ and $y_q$. Thus, $y_p$ is the fact while $y_q$ is one of its counterfactuals.


\subsection{Prompt-tuning Paradigm}
Since PLMs are mostly trained tasks in cloze-style, prompt tuning approach has been recently proposed to narrow the gap between downstream fine-tuning and pre-training tasks.
Formally, prompt tuning consists of the template $T(\cdot)$ and a verbalizer $\phi: \gV \rightarrow \gY$ that bridges the class set $\gY$ and the set of answer words $\gV$. 
Each class can be mapped to one or multiple answer words.
The templates include each token of original instance $x$ and additional tokens. 
The additional tokens can be discrete or continuous. 
Specifically, to construct the cloze-style tasks, at least one placeholder \texttt{[MASK]} should be placed into the template for the PLMs, $\gM$, for filling the valid words from the verbalizer. 
With the template $T(\cdot)$ and the verbalizer $\phi$, the learning objective is to maximize $\frac{1}{|\gX|} \sum_{x \in \gX} \log p(\texttt{[MASK]} = \phi(y_x)|T(x))$.
For example, for a binary sentiment classification, the template could be $T(x)=\{x$ It was \texttt{[MASK]}.\}.
Then it transforms $x$ into \{$x$ It was \texttt{[MASK]}.\} as the input of $\gM$. 
While for the verbalizer, the positive sentiment and the negative sentiment are respectively mapped to ``good'' and ``bad''. With the filling words selected by $\gM$, we can know whether the instance $x$ is positive or negative. We will extend this template in later sections.

